Beyond Invariance: Test-Time Label-Shift Adaptation for Distributions with "Spurious" Correlations

Changes in the data distribution at test time can have deleterious effects on the performance of predictive models $p(y|x)$. We consider situations where there are additional meta-data labels (such as group labels), denoted by $z$, that can account for such changes in the distribution. In particular, we assume that the prior distribution $p(y, z)$, which models the dependence between the class label $y$ and the "nuisance" factors $z$, may change across domains, either due to a change in the correlation between these terms, or a change in one of their marginals. However, we assume that the generative model for features $p(x|y,z)$ is invariant across domains. We note that this corresponds to an expanded version of the widely used "label shift" assumption, where the labels now also include the nuisance factors $z$. Based on this observation, we propose a test-time label shift correction that adapts to changes in the joint distribution $p(y, z)$ using EM applied to unlabeled samples from the target domain distribution, $p_t(x)$. Importantly, we are able to avoid fitting a generative model $p(x|y, z)$, and merely need to reweight the outputs of a discriminative model $p_s(y, z|x)$ trained on the source distribution. We evaluate our method, which we call "Test-Time Label-Shift Adaptation" (TTLSA), on several standard image and text datasets, as well as the CheXpert chest X-ray dataset, and show that it improves performance over methods that target invariance to changes in the distribution, as well as baseline empirical risk minimization methods. Code for reproducing experiments is available at https://github.com/nalzok/test-time-label-shift .

==> sections/abstract-old.tex <==
\begin{abstract}
\eat{
Spurious correlations, or correlations that change across domains where a model can be deployed, present significant challenges to real-world applications of machine learning models. However, such correlations are not always ``spurious''; often, they provide valuable prior information for a prediction. Here, we present a test-time adaptation method that exploits the spurious correlation phenomenon, in contrast to recent approaches that attempt to eliminate spurious correlations through invariance. 
}
Changes in the data distribution at test time can have deleterious effects on the performance of predictive models $p(y|x)$.
We consider situations where there are additional meta-data labels (such as group labels), denoted by $z$, that can account for such changes in the distribution. In particular, we assume that 
the prior distribution $p(y,z)$, which models the dependence between the class label $y$ and the ``nuisance'' factors $z$, may change across domains, either due to a change in the correlation between these terms, or a change in one of their marginals. However, we assume that the generative model for features $p(x|y,z)$ is invariant across domains. We note that this corresponds to an expanded version of the widely used
``label shift'' assumption, where the labels now also include the nuisance factors $z$. 
Based on this observation,  we
 propose a test-time label shift correction that adapts to changes in the joint distribution $p(y, z)$ using EM applied to unlabeled samples from the target domain distribution, $\ptarget(x)$.
 Importantly, we are able to avoid fitting a generative model $p(x|y,z)$,
 and merely need to reweight the outputs of a discriminative
 model $\psource(y,z|x)$ trained on the source distribution.
  We evaluate our method, which we call ``Test-Time Label-Shift Adaptation'' (TTLSA), on several standard image and text datasets, as well as the \chexpert chest X-ray dataset, 
and show that it improves performance over methods that target invariance to changes in the distribution,
as well as baseline
empirical risk minimization methods.
Code for reproducing experiments is available at \url{https://github.com/nalzok/test-time-label-shift}.
\end{abstract}

==> sections/old-methods.tex <==
\section{Test-Time Label Shift Adaptation}
We consider the following problem.
Given $\data_s^{xyz} = \{(\vx_n, y_n, z_n) \sim \psource(\vx, y, z)\}$ and $\data_t^{\vx} = \{\vx_n \sim \ptarget(\vx)\}$, we aim to construct a Bayes optimal predictor under the target domain, $f_t(\vx)$.
The core insight behind our method is that the optimal prediction for the class label in the target domain is given by 
\begin{equation*}
\begin{aligned}
f_t(\vx) =& \arg\max_y \ptarget(y|\vx) 
= \arg\max_y \sum_z \ptarget(y, z|\vx).
\end{aligned}
\end{equation*}
where $\ptarget(y,z|\vx)$ is given by Bayes' rule, as follows:
\begin{equation}
\label{eq:posterior}
\begin{aligned}
\ptarget(y,z|\vx) \propto
\ptarget(\vx|y,z) \ptarget(y,z) 
= \psource(\vx|y,z) \ptarget(y,z)  
\propto
\frac{\psource(y,z|\vx)}{\psource(y,z)}
\ptarget(y,z).
\end{aligned}
\end{equation}
Here, we use the assumption that $\ptarget(\vx|y,z) = \psource(\vx|y,z)$,
and the fact that
$\psource(y,z|\vx) \propto \psource(\vx|y,z) \psource(y,z)$.
(This latter fact lets us replace the generative model with a discriminative one;
this is known as the ``scaled likelihood trick'' \citep{Renals1994}.)

We make several observations.
First, \eqref{eq:posterior} is a simple reweighting of the unmodified source posterior $\psource(y, z|x)$, so we can apply this identity at test time.
Secondly, if we know the target prior $\ptarget(y,z)$, we can adapt any source posterior $\psource(y, z|\vx)$ to match any target $\ptarget(y, z|\vx)$, so long as $\psource(y, z)$ and $\ptarget(y,z)$ have common support.
%This gives us a degree of freedom in considering which source prior to target at training time.
Third, when we do not know the target prior $\ptarget(y,z)$, we can apply methods from the label shift adaptation literature to estimate this quantity using unlabeled samples from the target domain.
Finally, to apply \eqref{eq:posterior} in practice, we require that our model outputs behave like probability distributions; as such, calibration may be necessary.

Based on these observations, we propose the following procedure, which we call TTLSA:
\begin{enumerate}
\item Train a model $f_s(\vx)$ predicting $m=(y,z)$ taking $\vx$ as input using $\data_s^{xyz}$.
\item Estimate $\psource(y,z)$ empirically from $\data_s^{xyz}$.
\item Estimate $\ptarget(y,z)$ using $\data_t^{x}$ and a label shift adaptation identity.
\item Apply bias corrected temperature scaling (BCTS) to $f_s(\vx)$ to approximate $\psource(y, z|\vx)$.
\item Plug the results into \eqref{eq:posterior}.
\end{enumerate}

We discuss these steps in more detail below.

%We can estimate $\psource(y,z)$ empirically,
%since we assume we observe the meta-labels $m=(y,z)$ at training time. Similarly, we can fit $\psource(m|\vx)$ using any kind of discriminative classifier, such as a neural network or random forest. The only remaining challenge is estimate $\ptarget(y,z)$ from unlabeled samples from $\ptarget(\vx)$.
%We discuss how to do this below.

\subsection{Estimating the target prior from unlabeled data}

Given some unlabeled samples from the target distribution, $\data_t = \{ \vx_n \sim \ptarget(\vx): n=1:N \}$,
our goal is to estimate the prior on the meta-labels, $\ptarget(m)=\ptarget(y,z)$.
We will do this by maximizing the log likelihood,
$\mathcal{L}(\vx; \ptarget(m)) = \sum_{\vx_n} \log \ptarget(\vx_n)$,
where 
\begin{equation}
\begin{aligned}
\ptarget(\vx)
= \log\left(\sum_m 
\ptarget(m) \ptarget(\vx|m) \right) 
=  \log\left(\sum_m \ptarget(m) \frac{\psource(m|\vx)}{\psource(m)} \right)
+ \text{const}
\end{aligned}
\end{equation}

This objective is a sum of logs of a linear function of $\ptarget(m)$.
This needs to be maximized subject to the affine
constraints $\ptarget(m) \geq 0$ and $\sum_{m=1}^M \ptarget(m)=1$,
 so the problem is concave,
with a unique global optimum \citep{Alexandari2020},
implying the parameters are identifiable
\citep{Lipton2018,Garg2020shift}.

A simple  way to compute this optimum is to use EM,
which automatically satisfies the constraints.
Let $p_t^j(m)$ be the estimate of $\ptarget(m)$ at iteration $j$.
We initialize with $p_t^0(m) = \psource(m)$ and run the following iterative procedure below
(where we use the assumption
that $p_t(\vx|m)=p_s(\vx|m)$,
and Bayes rule to get
$p_s(m|\vx) = p_s(\vx|m) p_s(m) / p_s(\vx)$):
\begin{equation*}
\begin{aligned}
p_t^j(m|\vx_n) \propto& 
\ptarget(\vx_n|m) p_t^j(m)
\propto \frac{p_s(m|\vx)}{p_s(m)} p_t^j(m) \\
p_t^{j+1}(m) &=
\frac{1}{N} \sum_{n=1}^N
p_t^j(m|\vx_n)
\end{aligned}
\end{equation*}
This converges within a few iterations to the global maximum.
We can also modify this to compute a MAP estimate, instead of the MLE, by using a Dirichlet prior.
See Section~\ref{sec:em-deriv} in the Appendix for a detailed derivation.

\subsection{Calibration}
\label{sec:calibration}

Our unsupervised adaptation procedure crucially relies on the fact that the output of the classifier, $\psource(y,z|\vx)$, can be interpreted as calibrated probabilities.
Since modern neural networks are often uncalibrated
\citep[see, e.g.,][]{Guo2017-wm},
we have found it important to perform an explicit calibration step.
(See the appendix for an ablation study where we omit the calibration step.)

Specifically, we follow 
 \citet{Alexandari2020} and use the method they propose, known as  ``bias corrected temperature scaling'' (BCTS), which is a generalization of Platt scaling to the multi-class case.
In particular, let $l(\vx)$ be the vector of $M$ logits.
We then modify $\psource(m|\vx)$ as follows:
\begin{equation}
\psource(m |\vx) \propto \exp\left(\frac{l(\vx)_m}{T} + b_m\right)
\end{equation}
where $T \geq 0$ is a learned temperature parameter, and $b_m$ is a learned bias.
This calibration is done after the source classifier is trained.

\subsection{Choice of source distribution}
Although our focus here is test-time label shift adaptation, label shift adjustment can also be applied at training time.
This gives us a degree of freedom to consider which base posterior $p_s(y,z|\vx)$ to estimate at training time so that it can be most effectively adapted to any $p_t(y,z|\vx)$ via reweighting at test time.
A natural choice of source distribution, which we find to have some marginal benefit in practice, is the unconfounded distribution where $\psource(y,z) = \psource(y)\psource(z)$.
Thus, in our main implementation, we apply the logit adjustment strategy, described in Section~\ref{sec:logit}, at training time to the base classifier, and then apply TTLSA on top of this,
as though this were the true source distribution.
We note, however, that at a population level, this should make no difference.

\section{Invariant classifier baselines}

Although the focus of our paper is going beyond invariance, we still want a method for creating an invariant classifier to use as a baseline.
To approximate the optimal risk invariant predictor,
we take inspiration from Proposition 1 of
\citet{Makar2022},
which showed that a classifier that is trained on the unconfounded or balanced distribution $\pbalanced$, such that $\pbalanced(y,z) = p_s(y) p_s(z)$, will not learn any ``shortcut''
between the confounding factor $z$ and
the target label $y$.
Such a model will therefore have a risk which is invariant
to changes in the $p(z|y)$ distribution, and, in ``purely spurious'' anti-causal settings (a special case of Figure~\ref{fig:model}), they showed that this is indeed the optimal one among all risk-invariant predictors (see discussion in \cref{sec:related}).
We can simulate this optimal predictor by using any of
the methods we discuss below.
\eat{
the SUBG method (\cref{sec:SUBG})
or logit adjustment (\cref{sec:logit}).
We also note that GMTL  (\cref{sec:GMTL})
interpolates between the unadjusted $\psource$ model and a risk-invariant predictor, depending on $\alpha$.
}

\paragraph{SUBG adjustment}
\label{sec:SUBG}

%\todoqingyao{I'm not sure if SUBG belongs to Section 3, as it's just an invariance baseline, not an intermediate step in our proposed procedure. Maybe we should merge it with Section 3.3, or even move it to Section 2?}

%When fitting the classifier on the source domain, $\psource(y,z|\vx)$, the model may exploit ``shortcuts'', in which it predicts $z$  given $\vx$ and uses the correlation between $y$ and $z$ to predict $y$. For example, in the colored MNIST experiments in \cref{sec:cmnist}, it is easier for the model to learn to predict the color $z$, and exploit the fact that this is correlated with the class $y$, than it is to predict the class directly based on the shape of the digit. 
%Although our test time adaptation procedure can adapt to changes in the prior correlation, this approach will fail if the likelihood function $p(\vx|y,z) \propto p(y,z|\vx)$ ignores the dependence of $y$ on $\vx$.

%To prevent this from happening, we can train the classifier on a balanced version of the source data, in which there is no dependence between the class labels $y$ and the nuisance labels $z$.
A simple way to learn $\pbalanced(y | \vx)$ is to use the ``SUBG'' method of 
 \citep{idrissi2022simple}, which subsamples the data so there is an equal number of examples in each group $m=(y,z)$, then trains a classifier by standard ERM. 
 Despite its simplicity, they showed that this method yields SOTA results on various benchmarks.

 \paragraph{Logit adjustment}
\label{sec:logit}

 A downside of the SUBG method is that it discards data, thus reducing the amount of data available to train the classifier. Here, we propose a simple alternative, based on the logit adjustment idea of \citep{Menon2021}.
 %In more detail, suppose the target distribution did not suffer from spurious correlation,
 %so $\ptarget(y,z) = \ptarget(y) \ptarget(z)$.
 If both marginals $\pbalanced$ are uniform, then
 $\pbalanced(y,z) \propto 1$,
 so the corresponding balanced version of the source distribution becomes
$
\pbalanced(m|\vx) \propto \frac{\psource(m|\vx)}{\psource(m)}
$,
which in log space becomes
$\log(\pbalanced(m|\vx)) \equiv
\log(\psource(m|\vx)) - \log(\psource(m))$.
We can fit the balanced source domain classifier by optimizing the above objective on the labeled training set.
After fitting, we can recover the original source domain classifier using
$\psource(m|\vx) \propto \pbalanced(m|\vx) \psource(m)$.
Note that when the marginals are not uniform, one can apply a similar adjustment, subtracting off $\log(\psource(y,z) / (\psource(y)\psource(z)))$.

%\todoqingyao{We should mention TTSLA on Logit Adjustment works better than TTSLA on Unadapted.}


\eat{
In practice, we find it yields higher predictive accuracy if we use a logit adjusted softmax cross-entropy loss to estimate the invariant posterior $\pbalanced(m|\vx)$ and then adapt it to the target domain, i.e.
\begin{equation}
\begin{aligned}
\pbalanced(m|\vx) \propto& \frac{\psource(m|\vx)}{\psource(m)} \\
\ptarget(m|\vx) \propto& \pbalanced(m|\vx) \ptarget(m)
\end{aligned}
\end{equation}

\todo{clarify the difference between ``targeting invariance at training time'' and ``training normally and subtract a margin from the logit output'', and explain why the former works better (something related to encouraging the network to focus on the minority class?)}

While this is mathematically equivalent to Equation~\eqref{eq:posterior} at the population level, in practice an intervention at training time makes things work better.
Additionally, note that post-hoc logit adjustment results in only $\psource(m|\vx)$ being calibrated, whereas $\psource(m)$ is estimated separately on the training set.
However, if we train with a logit-adjusted loss to estimate $\pbalanced(m|\vx)$ directly, then $\psource(m|\vx)/\psource(m)$ is calibrated on the validation set as a whole, which partially explains its superior performance.

}


\eat{
\subsection{GMTL baseline}
\label{sec:GMTL}

The GMTL or 
 ``generative multi-task learning'' approach of \citet{Makino2022} is closely related to the approach in our paper.
 However, instead of estimating $\ptarget(y,z)$ from unlabeled data,
 they just assume that 
 $\ptarget(y,z) \propto \psource(y,z)^{1-\alpha}$ for some value of $\alpha$.
They do not give a procedure for estimating $\alpha$, but instead report results for across the range $\alpha \in [0,1]$.
Note that setting  $\alpha=1$,
recovers an invariant classifier,
similar to logit adjustment and SUBG.
Also, setting $\alpha=0$ recovers a standard
unadapted model.
For values of $\alpha$ in between 0 and 1,
the results lie between the unadapted model and the invariant model.
%, as we show in the appendix.
}

==> sections/results/ablation.tex <==

\subsection{Ablation studies}
\label{sec:ablation}



In this section, we study various ablations to our method, focusing on the \chexpert dataset.
(The findings are qualitatively similar on the \cmnist dataset.)

In \cref{fig:chexpert-embedding-domain1-cali},
we show the results of our method using target datasets of size $N=64$ and $N=512$.    We see that the larger sample size improves estimation of the target meta-label prior, and brings TTLSA closer to the oracle.

In \cref{fig:chexpert-embedding-domain1-nocali} we show the results if we remove the calibration step.
Compared to \cref{fig:chexpert-embedding-domain1-cali},
we see that the overall AUC of all the methods is worse, and the variance is larger.
\footnote{
%
For a binary classification problem, calibration will not change the AUC, but since we derive the posterior over class labels by marginalizing a 4-way joint,
$p(y|\vx) = \sum_{z=0}^1 p(y,z|\vx)$,
calibration can help.
}
However, the rank ordering of the methods is the same.
It is notable that a large gap opens up between the Oracle curve and the TTLSA implementations.
This suggests that calibration primarily improves estimation of $\ptarget(y,z)$ estimation via EM, because the Oracle curve in this subfigure corresponds to using the correct weights with the uncalibrated $\psource(y,z|\vx)$ model.








==> sections/results/mimic.tex <==
\subsection{MIMIC-CXR}

We conducted a similar experiment on MIMIC-CXR.

==> sections/results/synthetic.tex <==
\subsection{Synthetic data}

We first evaluate our method on some "toy" datasets, to better understand its behavior.
